Scheduling for Multi-Phase Parallelizable Jobs

With multiple identical unit speed servers, the online problem of scheduling jobs that migrate between two phases, limitedly parallelizable or completely sequential, and choosing their respective speeds to minimize the total flow time is considered. In the limited parallelizable regime, allocating $k$ servers to a job, the speed extracted is $k^{1/\alpha}, \alpha>1$, a sub-linear, concave speedup function, while in the sequential phase, a job can be processed by at most one server with a maximum speed of unity. A LCFS based algorithm is proposed for scheduling jobs which always assigns equal speed to the jobs that are in the same phase (limitedly parallelizable/sequential), and is shown to have a constant (dependent only on $\alpha > 1$) competitive ratio. For the special case when all jobs are available beforehand, improved competitive ratio is obtained.

==> Equiv-ParallelSlowdown-SpeedScaling.tex <==
\section{Equivalence between the parallel scheduling model of heSRPT
  and speed scaling with net power constraint}

We use the notation from [heSRPT]: $N$ parallel and identical servers,
$M$ jobs. Size of job~$i$ is $x_i.$ Let $k_i$ denote the `number' of
servers alloted to job~$i,$ then the service rate experienced by
job~$i$ is $s_i = S(k_i) = k_i^p,$ where $p \in (0,1).$ Here,
$S(\cdot)$ denotes the speedup function. Note that
$\sum_{i = 1}^M k_i \leq N.$

Equivalently, suppose that each job has its own (solo) server, and let
$s_i$ denote the speed allocated to the server processing job~$i$
(note that each job can be allocated a non-zero speed, which makes
this an infinite server model). Interpret
$k_i = P(s_i) := S^{-1}(s_i)$ as the power consumption of job~$i.$
Note that $P(s) = s^{1/p}$ is convex increasing. Thus, the constraint
$\sum_{i=1}^M k_i \leq N$ becomes
$$\sum_{i=1}^M P(s_i) \leq N,$$ which can be thought of as a total
power constraint.

In both interpretations, the service speed of job~$i$ is $s_i,$ so the
flow times across both would be identical.


==> PotentialFunction.tex <==
\section{System Model}
\subsection{FCFS}
Consider a single server following a FCFS discipline for scheduling jobs. Job $j$ with size $w_j$ arrives at time $t_j$ and jobs are processed in order of their arrival sequence. Server uses speed $s(t)$ at time $t$ and consumes power $P(s(t))$. The objective is to minimize the flow time (summed across jobs) + energy (summed across time).  

Consider the following locally optimal speed scaling algorithm, that chooses speed $s(t)$ at time $t$
\begin{equation}\label{eq:speeddef}
 s(t) = P^{-1}\left(n(t)\right),
 \end{equation}
 where $n(t)$ is the number of outstanding jobs at time $t$. This is infact optimal assuming no further jobs are going to arrive in future.



{\bf Lower Bound} We first show that the locally optimal speed scaling algorithm \eqref{eq:speeddef} has competitive ratio $\Omega(n^{1/\alpha})$ where $n$ is the total number of jobs in the input. 
To do so, consider the following input. 
At time $0$, a job $1$ with size $w$ arrives. Algorithm \eqref{eq:speeddef} will process this job at speed $1$. Starting from time $w/2+k$, $k=0, \dots, w^{\frac{\alpha}{\alpha+1}}$, a single job with size $1$ arrives for each $k$. The algorithm chooses 
speed $k^{1/\alpha}$ between time instants $w/2+k$ and $w/2+k+1$, $k=0, \dots, w^{\frac{\alpha}{\alpha+1}}$ for job $1$. 
Thus, the amount of work done on job $1$ between time instants $w/2+k$ and $w/2+k+1$ for $k=0, \dots, w^{\frac{\alpha}{\alpha+1}}$ is $k^{1/\alpha}$, and total work remaining for job $1$ at time $w/2$ is $w/2$. 
Thus, job $1$ is completed at time $\frac{w}{2}+ \frac{w^{\frac{\alpha}{\alpha+1}}}{2}$. Therefore the job arriving at time $\frac{w}{2}+k$, $k=0, \dots, w^{\frac{\alpha}{\alpha+1}}$ has to wait for time at least $\frac{w^{\frac{\alpha}{\alpha+1}}}{2} - k$ before it can be processed. 
Therefore, the total flow time (counting only the wait times for jobs arriving at time $w/2+k$, $k=0, \dots, w^{\frac{\alpha}{\alpha+1}}$, is at least $\frac{w^{\frac{\alpha}{\alpha+1}}}{2}(\frac{w^{\frac{\alpha}{\alpha+1}}}{2}+1)/2 = \Omega(w^{\frac{2\alpha}{\alpha+1}})$, letting $w$ to be large. 

Now we consider an alternate algorithm to lower bound the flow time + energy for the $\opt$. Consider the speed choice for time $0$ till $w/2$ as $2$ and thereafter speed $1$ throughout. With this speed choice, no incoming job has to wait behind any other job. The total flow time + energy for job $1$ is $w/2 + 2^\alpha w/2$ while for the unit sized job is $2$. Thus, the total flow time + energy for all jobs is $2w^{\frac{\alpha}{\alpha+1}}+ (2^\alpha+1) w$.

Therefore the competitive ratio of the speed scaling algorithm \eqref{eq:speeddef} is $\Omega(w^{\frac{\alpha-1}{\alpha+1}})$. Since the number of jobs $n=w^{\frac{\alpha}{\alpha+1}}+1$, we get that the competitive ratio is at least $\Omega(n^{\frac{\alpha-1}{\alpha}})$.

The same bound can be shown for any other speed scaling algorithm that is online, by suitably changing the input since the algorithm \eqref{eq:speeddef} is locally optimal under the causal information about the input 
that an online algorithm can have.

{\bf Upper Bound}
Next, we show an upper bound on the competitive ratio for the speed scaling algorithm \eqref{eq:speeddef} as $O(n^{1-1/\alpha})$ matching the lower bound. Towards that end,  consider the following potential function. Let $A(t)$ be the set of outstanding jobs with the algorithm at time $t$, ${\hat w}_j(t)$  be the remaining size of the job $j$ at time $t$ with the algorithm, and $n([t_j, t])$ be the number of outstanding jobs with algorithm 
 that have arrived between time $t_j$ (arrival time of job $j$) and $t$. 

\begin{equation}
  \label{eq:phi}
  \Phi(t) = \frac{c}{\alpha} \sum_{j\in A(t)} \Delta(n_A([t_j, t])) {\hat w}_j(t)  
  \end{equation}
  where $(x)^+ = \max\{x,0\}$, and $\Delta(x) = P^{'}(P^{-1}(x))$.


% The quantity $f(1)$ will show up in the bound on the competitive
% ratio.  For $P(x) = x^\alpha$, $f(1) = \alpha$.
%
% For $\alpha \ge 2$, this implies that $f(x)$ is strictly
% convex. Thus $k f(x/k) \ge (k+1)f(x/(k+1))$, which we will use later
% on to bound the jumps of the potential function $\Phi(t)$ Define
% $\Delta(i) = 0$ for $i \leq 0.$ %\jk{Move to appendix.}

%{\bf Algorithm: } The speed scaling algorithm that we propose, chooses
%the following speed for the server,
 

 

\begin{lemma}\label{lem:jump}
  The total increase in $\Phi(\cdot)$ at
  points of discontinuity is at most $c n^{1-1/\alpha} \sum_{j=1}^n w_j$.
\end{lemma}

\begin{proof}
Function $\Phi(t)$ can have discontinuities only when either a job arrives into the system or leaves the system. 
First consider the arrival of new job $j$ at time $t_j$. On any arrival, $n_A([t_k, t] = n_A([t_k, t]+1$ for $t_k\le t_j$, increasing the potential function by $\frac{c}{\alpha} \Delta((n_A([t_k, t]+1) - \Delta((n_A([t_k, t]) w_k$ for the  job $k \in A(t)$. 
Thus for any job $k$ among the total $n$ jobs, the maximum increase in $\Phi(.)$ can be 
$\frac{c}{\alpha}  \sum_{j=1}^n \Delta((n_A([t_j, t]+1) - \Delta((n_A([t_j, t]) w_k 
\le \frac{c}{\alpha}  \Delta(n) w_k \le c n^{1/\alpha} w_k$, since $\Delta(n) = P'(P^{-1}(x)) = \alpha x^{1-1/\alpha}$. Thus, summing over all jobs, we get 
that the total increase in $\Phi(\cdot)$ at all arrival instants is $\sum_{k=1}^n c n^{1-1/\alpha} w_k $. 

Clearly, when a job departs, ${\hat w}_j(t) =0$, thus $\Phi(\cdot)$ does not change.



\end{proof}


Let $n(t)$ ($n_o(t)$) be the total outstanding jobs with the algorithm ($\opt$) at time $t$ and $s_o(t)$ be the speed of the $\opt$ at time $t$. Then we have the following result for the drift of potential function $\Phi(t)$. 
\begin{lemma}\label{lem:drift}
  $$d\Phi(t)/dt  \le \frac{c}{\alpha}\Delta(n(t)) (-s(t)).$$
\end{lemma}
\begin{proof}

The algorithm will be working on its earliest active arrived job $j$ (at rate $-s(t)$) that arrived at time $t_j$, and
 $n([t_j,t] = n(t)$.
Hence the contribution in $d\Phi(t)/dt$ from the algorithm is 
$d\Phi(t)/dt = - \Delta(n(t)) s(t)$, as needed.

\end{proof}

The main theorem of this paper is as follows.
\begin{theorem}\label{thm:main}
  The proposed speed scaling algorithm \eqref{eq:speeddef} is
  $2\alpha n^{1-1/\alpha}$-competitive for a single server following FCFS discipline.
\end{theorem}
To prove Theorem \ref{thm:main} we will require the following technical Lemma from
\cite{bansal2009speedconf}.
\begin{lemma}\label{lem:bansal}[Lemma 3.1 in~\cite{bansal2009speedconf}]
  For $s, {\tilde s}, \beta \ge 0$, then for any function $P$ that is
  strictly increasing, strictly convex, and differentiable,
\begin{align*}
\Delta(\beta)(-s + {\tilde s}) \le& \left(-s +P^{-1}(\beta)\right)P^{'}(P^{-1}(\beta)) 
%\label{eq:powerbound}
 + P({\tilde s}) -\beta.
\end{align*}
\end{lemma}
\begin{proof}
Let $n(t) \le n_o(t)$, then upper bounding $d\Phi(t)/dt$ by $0$, the running cost $n(t) + P(s(t)) + d\Phi(t)/dt$ 
\begin{align*} 
& \le n(t) + n(t) \\
& \le 2 n_o(t).
\end{align*}
When 
Consider the running cost $n(t) + P(s(t)) + d\Phi(t)/dt$ 
\begin{align*} 
& \le n(t) + n(t) - \frac{c}{\alpha} (-s(t) + P^{-1}(n(t)) P'(P^{-1} (n(t)))\\
& \quad  - (n(t) )),\\
& \le n(t) + n(t) - \frac{c}{\alpha} n(t), \\
& \le 0,
\end{align*}
where $(a)$ follows from Lemma \ref{lem:drift} and using Lemma \ref{lem:bansal}, $(b)$ follows since $s(t) = P^{-1}(n(t))$, and $(c)$ follows by choosing $c=2\alpha$.
Thus, in both cases we have shown that \eqref{eq:mothereq} holds for $c=2\alpha$.
\end{proof}


\begin{comment}
\begin{proof} From Lemma \ref{lem:costwithjump}
\begin{align}\label{eq:res1}
C_A \le 6C_{\opt} +12 nK f(1),
\end{align}
by choosing $c_i=6$ for all servers.
For any job with size $w$, the minimum cost incurred by $\opt$ on processing it on any one server is 
$\min_s \frac{w}{s}+\frac{wP(s)}{s}$, where $s$ is the speed. Thus, the optimal $s^\star$ satisfies $1+P(s^\star)= s^\star P'(s^\star)$, and the optimal cost is  $wP'(s^\star)$.
For $P(s) = s^2$, $s^\star =1$ and the minimum cost is $2$ for $w=1$. 
With $n$ jobs arriving each with size $1$ which have to be processed by each of the $K$ servers, a simple lower bound on the cost of $\opt$ is $2nK$. This implies from \eqref{eq:res1} that 
\begin{align}\label{eq:res11}
C_A & \le 6C_{\opt} + 6C_{\opt} f(1) = C_{\opt}6(1+f(1)).
\end{align}
\end{proof}
\begin{definition}\label{defn:r}
Let $r_i=\ell$, if $i$ is the $\ell^{th}, \ell \in [1:A(t)]$ active server (in increasing order of server index) among the $A(t)$ active servers.
\end{definition} 
The proof of Theorem~\ref{thm:main} is based on the following bounds
on the potential function drift. \begin{lemma}\label{lem:bansalphi1}
When $n^1(t)>0$, for any active server $i$
\begin{align*}d\Phi_i/dt\le  c_i P(s_i^o) - c_i \frac{n^1(t) + r_i}{A(t)} + c_i \frac{n^1_o(t) + \sum_{k=2}^{i}\b1^k_o(t) n^k_o(t)}{A(t)},  
\end{align*}
where $\b1^i_o(t)=1$ if server $i$ is active with the $\opt$ and $0$ otherwise,
and $d\Phi_i/dt = 0$ for any inactive server.
When $n^1(t)=0$, for any active server $i$
$$d\Phi_i(t)/dt  = c_i\left(P(s_i^o) - c_i \frac{ r_i}{A(t)} + c_i \frac{n^1_o(t) + \sum_{k=2}^{i}\b1^k_o(t) n^k_o(t)}{A(t)} \right),$$ and $d\Phi_i/dt = 0$ for any inactive server.

\end{lemma}
\begin{lemma}\label{lem:costwithjump}
$C_A \le 6C_{\opt} + 12 nK f(1)$.
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:costwithjump}]
We show that for any time $t$ where $\Phi$ is differentiable, $n(t)+ \sum_{i\in A(t)}P(s_i) + d\Phi/dt  \le 6  (n_o(t) + \sum_{i=1}^K P(s_i^o))$.
Combining this with Lemma \ref{lem:jump} (choosing $c=6$), we get that 
 $C_A \le \int \left(n(t)+ \sum_{i\in A(t)}P(s_i)\right)dt + \int d\Phi/dt  dt \le 6   \int (n_o(t) + \sum_{i=1}^K P(s_i^o))dt + 12 nK f(1)$. Since 
 $\int (n_o(t) + \sum_{i=1}^K P(s_i^o))dt = C_{\opt} $, we get the result.

We first consider the case when server~$1$ is busy, i.e. $n^1(t) > 0$.
\begin{enumerate}
\item Subcase I:  $n^1(t) > 0$: 
From Lemma \ref{lem:bansalphi1}, we get 
$n(t)+ \sum_{i\in A(t)}P(s_i) + d\Phi/dt $
\begin{align*} &= n^1(t)  + A(t)-1 + \sum_{i\in A(t)}P(s_i) + d\Phi/dt\\
& \stackrel{(a)}= n^1(t)  + A(t)-1   +\sum_{i\in A(t)}P\left(P^{-1}\left(\frac{n^1(t)+A(t)}  {A(t)}\right)\right) \\
& \ \ \ \ \ 
+ \sum_{i\in A(t)}c_i P(s_i^o) - c_i \sum_{i\in A(t)}\frac{n^1(t) + r_i}{A(t)} + c_i \sum_{i\in A(t)}\frac{n^1_o(t) + \sum_{k=2}^{i}\b1^k_o(t) n^k_o(t)}{A(t)}, \\
&\stackrel{(b)}\le 2(n^1(t)  + A(t))-1 -  \sum_{i\in A(t)} c_i \frac{n^1(t) + r_i}{A(t)}  +  \sum_{i\in A(t)}c_i P(s_i^o)  + c_i \sum_{i\in A(t)}\frac{n_o(t)}{A(t)} , \\
&\stackrel{(c)} \le (2 - c_i)n^1(t)-1 + (2 - c_i/2) A(t) + c_i/2 + \sum_{i\in A(t)}c_i P(s_i^o) +  c_i n_o(t)
\end{align*}
where $(a)$ follows by plugging in the speed definition \eqref{eq:speeddef} and using Lemma \ref{lem:bansalphi1}, $(b)$ follows since $n^1_o(t) + \sum_{k=2}^{i}\b1^k_o(t) n^k_o(t) \le n_o(t)$, 
and $(c)$ follows since $\sum_{i\in A(t)} \frac{n^1(t) + r_i}{A(t)} \ge n^1(t)  + \frac{A(t)-1}{2}$ by definition of $r_i$.
Thus, choosing $c_i=4$ for all servers $i$, we get 
$$n(t)+ \sum_{i\in A(t)}P(s_i) + d\Phi/dt  \le 4  ( n_o(t) + \sum_{i=1}^K P(s_i^o) ),$$ as required.
\item Subcase II:  $n^1(t) = 0$: In this case, From Lemma \ref{lem:bansalphi1}, we get 
$n(t)+ \sum_{i\in A(t)}P(s_i) + d\Phi/dt $
\begin{align*} &=  A(t) + \sum_{i\in A(t)}P(s_i) + d\Phi/dt,\\
& \stackrel{(a)}=  A(t)   +\sum_{i\in A(t)} P\left(P^{-1}(2)\right) 
+ \sum_{i\in A(t)} c_i\left(P(s_i^o) - \frac{ r_i}{A(t)} +  \frac{n^1_o(t) + \sum_{k=2}^{i}\b1^k_o(t) n^k_o(t)}{A(t)} \right), \\
&\stackrel{(b)}\le 3A(t) -  \frac{c_i}{A(t)}\sum_{i\in A(t)}  r_i  +  \sum_{i\in A(t)}c_i P(s_i^o)  + c_i n_o(t), \\
&\stackrel{(c)} \le (3 - c_i/2)( A(t)) -c_i/2+ \sum_{i\in A(t)}c_i P(s_i^o) +  c_i n_o(t),
\end{align*}
where $(a)$ follows from speed definition \eqref{eq:speeddef} of $s_i = P^{-1}(2)$ when $n^1(t) = 0$, $(b)$ follows since
$n^1_o(t) + \sum_{k=2}^{i}\b1^k_o(t) n^k_o(t) \le n_o(t)$, and $(c)$ from $\sum_{i\in A(t)} \frac{ r_i}{A(t)} \ge  \frac{A(t)+1}{2}$
Thus, choosing $c_i=6$ for all servers $i$, we get 
$n(t)+ \sum_{i\in A(t)}P(s_i) + d\Phi/dt  \le 6  (n_o(t) + \sum_{i=1}^K P(s_i^o) )$ as required.
\end{enumerate}
\end{proof}
\end{comment}

%\begin{enumerate} \item new arrival, no change since .  to server 1,
%$\Phi_1$ does not increase because both $n^1(t,q)$ and $n^1_o(t,q)$
%increase by $1$ for $q \in [0, q_a]$ where $q_a$ is the size of the
%newly arriving job. While $\Phi_2$ does not increase since the
%increase in $n^1(t,q)$ for $q \in [0, q_a]$ is compensated by
%increase in $n^1(q_{min})$, since $q_{min}\le q_a$.  \item departure
%from server 1 or server 2, only affects one point in integral at
%$q=0$, so no change.  \item departure from $s^2$, $n^2(q_{min})$ does
%not change, while $n^2(t)$ decreases by $1$ while $n^2(q,t) $ via the
%integral over $q$ is affected only for $q=0$. So the change in
%$\Phi_2$ is negative.



==> ProblemFormulation.tex <==
\section{System Model}\label{sec:sysmodel}
Let there be $N$ parallel and identical servers, each with speed $1$. The set of jobs is denoted by $\cJ$, where a job $j \in \cJ$ arrives at time $a_j$. Similar to \cite{edmonds2000scheduling, berg2019hesrpt}, we consider the continuous allocation model, where $N$ is treated as a single resource block which can be divided into chunks of arbitrary sizes and allocated to different jobs.

Each job $j$ at any time can be in one of two phases, called elastic or in-elastic. The sizes of job $j$ in the $a^{th}$ elastic and $b^{th}$ in-elastic phase are $w_{je}^a$ and $w_{j\iota}^b$, respectively. Moreover, let $A_j$ and $B_j$ be the total number of elastic and in-elastic (interleaved) phases required for each job, respectively. The first and the last phase of any job  can be either of the two phases. We consider the online setting, where an algorithm has only causal information about jobs, i.e. any job's phases and their respective sizes are revealed only once it arrives. 


In the elastic phase, any job is parallelizable with concave speedup, i.e.,  if job~$j$ is allotted 
$k_j(t)$ number of
servers at time $t$, then the service rate experienced by
job~$j$ at time $t$ is $s_j(t) = P(k_j(t)) = k_j(t)^{1/\alpha},$ where $\alpha > 1$.
%\footnote{This definition is a slight deviation from the speed function defined earlier $s(k) = k^{1/\alpha}$, however, is made for notational simplicity.}. 
Since we are considering the continuous allocation model, $k_j(t) <1$ is possible. Similar to \cite{berg2019hesrpt, vazeperf2021, berg2021case}, we let $s(k) = k_j(t)^{1/\alpha}$ even when $k_j(t) <1$.
%\begin{equation}\label{eq:serverconst}
%\sum_{j= 1}^{A(t)} k_j(t) \leq P^{-1}(N) \quad \text{or} \quad \sum_{j= 1}^{A(t)} P(s_j(t)) \leq N, 
%\end{equation} where $A(t)$ is the set of jobs that are being processed at time $t$.

In the in-elastic phase, each job can be processed by at most one server, and equivalently can be processed at speed of at most $1$. 
Moreover, for any job $j$, it transitions from the elastic to in-elastic phase or vice versa only when its total work $w_{je}^a$ or $w_{j\iota}^b$ in the current phase is complete.

A job $j$ is defined to be complete at time $d_j$, if $d_j$ is the earliest time at which total $\sum_{a\le A_j} w^a_{je} + \sum_{b \le B_j} w^b_{j\iota}$ amount of work has been completed for job $j$, and the objective is to minimize the flow time 
\begin{equation}\label{eq:flowtime}
\min F = \sum_{j\in \cJ} (d_j-a_j) =  \int n(t) dt \ \text{s.t.} \ \sum_{j= 1}^{A(t)} P(s_j(t)) \leq N,
\end{equation}
 where $n(t)$ is the number of outstanding jobs at time $t$, and  $A(t)$ is the set of jobs that are being processed at time $t$.
 
 
% Compared to our general system model, recently in \cite{berg2021case}, a three state Markov chain was considered for phase transitions as shown in Fig. \ref{fig:BD}, where each job arrives in either 
% the elastic or the in-elastic phase, and transitions between the two phases at fixed rates, and always exits from the in-elastic phase. Because of these strong assumptions, \cite{berg2021case} was able to identify an optimal policy that always prioritizes the jobs for scheduling that are in their in-elastic phases. With the general system model, this is no longer true, and in Section \ref{sec:algo}, we present a different algorithm and show that its competitive ratio is a constant.
% 
% \begin{figure}[h]
%\centering
%\begin{tikzpicture}[level/.style={sibling distance=50mm/#1}]
%\node[circle,draw] (s) at (0,0) {$E$};
%\node[circle,draw] (a) at (2,0) {$I$};
%\node[circle,draw] (b) at (4,0) {$C$};
%%\node[circle,draw] (c) at (6,0) {$3$};
%
%\draw[bend right, dashed,<-]  (s) to node [below] {$ p \lambda_E$} (a);
%\draw[bend right, dashed,<-]  (a) to node [above] {$\lambda_I$} (s);
%
%
%%\draw[bend right, dashed,<-]  (a) to node [below] {$\mu_2$} (b);
%\draw[bend right, dashed,<-]  (b) to node [above] {$(1-p) \lambda_E$} (a);
%
%
%%\draw[bend right, dashed,<-]  (b) to node [below] {$\mu_3$} (c);
%%\draw[bend right, dashed,<-]  (c) to node [above] {$\lambda$} (b);
%
%%\draw[dotted,thick]  (7,0) to node [above] {} (9,0);
%
%%\draw[bend right, dashed,->]  (a) to node [left] {$\lambda$} (s);
%%\draw[bend right, dashed,->]  (a) to node [left] {$\lambda$} (s);
%
%%\draw[bend right,dashed, ->]  (s) to node [below] {jump edge} (a);
%%\node [circle,draw] (s){$s$} at (0,0);
%%\node  [circle,draw] (a){$a$} at (0,2);
%%\node  [circle,draw] (b){$b$} at (1,1);
%%\path[-]  (s)    edge  node[sloped, anchor=center, below] {$3$}     (a);
%%\path[-]  (s)    edge  node[sloped, anchor=center, above] {$2$}     (b);
%%\path[-]  (a)    edge  node[sloped, anchor=center, above] {$10$}     (b);
%\end{tikzpicture}
%\caption{Birth death chain for phase evolution, where $I, E, C$ represent the in-elastic, elastic and completion phases, respectively, and $\lambda$'s are the transition rates, and $0 < p < 1$ is constant.}
%\label{fig:BD}
%\end{figure}
%
%For ease of exposition, equivalently, we consider the following speed scaling problem. Suppose that for each job we can `create'
%its own dedicated server, i.e., there are unlimited number of servers and a job is processed on only one server, and cannot be parallelized.
%Let $s_j(t)$ denote the speed allocated to the server processing job~$j$ at time $t$. If job $j$ is in its in-elastic phase, then $s_j(t)\le 1$.
%%Since there is no limit on the number of jobs available at any time, essentially, we are making this as an infinite server model. 
%Let 
%$k_j(t) = P(s_j(t)) := S^{-1}(s_j(t))$ be the power consumption of job~$j$ on its own server if it is processed at speed $s_j(t)$, where $P(s) = s^{\alpha}, \alpha>1$ is a convex increasing function. Then, \eqref{eq:serverconst} is equivalent to 
%$\sum_{j \in A(t)} P(s_j(t)) \leq N$,  the total
%power used across all the active servers is at most $N$.
%
%In both these models, the service speed of job~$j$ is $s_j,$ so the
%flow times across both the models would be identical. Thus, with this (infinite server speed scaling model) the equivalent objective is 


%\section{A more general problem formulation}
%Compared to Problem \eqref{eq:flowtime}, we consider a more general problem, as described next. Let there be an infinite supply of servers, however, any job can be processed on any one server at any time (no parallelization is allowed). We consider that preemption  is allowed, i.e., a job can be halted at any time, and restarted later on its own server.
%Each server when executing a job at speed $s(t)$ at time $t$, consumes power $P(s(t))$. Let $P(x) = x^\alpha$ where $\alpha > 1$. In addition, there is a sum-power constraint of $N$ across all servers, i.e., $\sum_{i : s_i(t) > 0} P(s_i(t)) \le N$, for all $t$, where $s_i(t)$ is the speed of an active server $i$ at time $t$. 
% 
%If a server works with speed $s$ for a time duration $t$ on a job, then $st$ amount of work is completed for that job.
%Set of jobs $J$ arrive over time, where an arriving job $j \in \cJ$ with size $w_j$ is defined to be complete at time $d_j$, if $w_j$ amount of work has been completed for it by time $d_j$, where the work could have been done over different servers at different times. Hence the flow time is $\sum_{j\in J} (d_j-a_j) = \int n(t) dt$, where $n(t)$ is the number of unfinished jobs in the system at time $t$.
%
%The metric of interest is the flow time + energy, $\int n(t)dt  + \int \sum_{i : s_i(t) > 0} P(s_i(t)) dt$,
%and the problem to solve is
%\begin{align}\label{eq:flowtimeplusenergy}
%\min  \int n(t)dt  + \int \sum_{i : s_i(t) > 0} P(s_i(t)) dt, \quad \text{subject to} \ \sum_{i : s_i(t) > 0} P(s_i(t)) \le N. &
%\end{align}
%\begin{remark} Note that even under the sum power constraint, the metric of flow time + energy is meaningful, since it is not necessary that the energy used by an optimal algorithm is equal to the maximum possible allowed by the constraint. For example, when the number of outstanding jobs is small, an optimal algorithm may choose a small speed such that the total power consumed is less than the sum-power constraint.
%\end{remark}
%
%Compared to Problem \eqref{eq:flowtime}, Problem \eqref{eq:flowtimeplusenergy} is more general, where we are minimizing the sum of flow time and energy under the sum-power constraint, with $N = N$ for Problem \eqref{eq:flowtime}. In the following, we will consider Problem \eqref{eq:flowtimeplusenergy}, and propose algorithms and bound their competitive ratios \eqref{defn:cr}. Minimal changes to be made for algorithms to be feasible, and analysis to be applicable for Problem \eqref{eq:flowtime} are mentioned in Remark \ref{rem:prob1}. Consequently, we will only indicate the corresponding competitive ratio results for Problem \eqref{eq:flowtime}.
%
\section{Metric}
We represent the optimal offline algorithm (that knows the entire job arrival sequence including the number of phases, and the respective sizes of jobs in each phase,  in advance) as $\opt$. 
Let $n(t)$ ($n_o(t)$)  be the number of outstanding jobs with an online algorithm $\cA$ ($\opt$). 
For Problem \eqref{eq:flowtime}, we will consider the metric of competitive ratio which for an online algorithm $\cA$ is defined as 
\begin{equation}\label{defn:cr}\mu_\cA  = \max_\sigma \frac{\int n(t)  dt}{\int n_o(t) dt},
\end{equation}
where $\sigma$ is the input sequence consisting of jobs set $\cJ$. 

We will propose an online algorithm $\cA$, and bound $\mu_\cA \le \kappa$, by showing that for each time instant $t$
\begin{align}\label{eq:runcond}
  n(t) +  d\Phi(t)/dt & \le \kappa  n_o(t),
\end{align}
where $\Phi(t)$ is some function called the {\bf potential function} that satisfies the boundary conditions:
\begin{itemize}
\item $\Phi(t) = 0$ initially before all job arrivals and $\Phi(\infty) = 0$.
\item $\Phi(t)$ does not increase on any job arrival or job departure with the algorithm or the $\opt$.
\end{itemize}
Integrating \eqref{eq:runcond} over time, implies that the competitive ratio of $\cA$ is at most $\kappa$.



\section{Algorithm \textsc{Fractional-LCFS}}\label{sec:algo}
%We first consider the case when $N \ge \frac{P(4)}{4}$.
In this section, we propose an algorithm that is semi non-clairvoyant, that disregards the information about the remaining job sizes of all the remaining phases, and only exploits the binary information about a job being in the elastic or the in-elastic phase, which will be compared against a clairvoyant optimal offline algorithm in terms of the competitive ratio.
At time $t$, let the outstanding number of jobs in the system be $n(t)$, and $n_\iota(t)$ be the number of jobs that are in their in-elastic phase. 
Thus, $n(t) = n_e(t)+ n_\iota(t)$, where $n_e(t)$ is the number of jobs that are in their elastic phase.

{\bf Scheduling and speed selection:} 
Let $\beta, \theta$ be constants with $0 < \theta < \beta < 1$.

Case I $\frac{N}{\beta n(t)} \le 1$: Process the $\beta n(t)$ jobs that have arrived {\bf most recently} without distinguishing between jobs that are in their elastic or in-elastic phase. \footnote{If $\beta n(t)$ is fractional, then we mean $\lceil \beta n(t) \rceil$.}  
{\bf Speed:} Each of the $\beta n(t)$ jobs are processed at equal speed 
\begin{align}\label{}
  s(t) & = P\left(\frac{N}{ \beta n(t)}\right).
\end{align}

Case II $\frac{N}{\beta n(t)} > 1$: 
IIa: If $n_\iota(t) \ge \theta n(t)$\footnote{If $\theta n(t)$ is fractional, then we mean $\lceil \theta n(t) \rceil$.} then process any $\min\{n_\iota(t),N\}$ jobs\footnote{If $N=\min\{n_\iota(t),N\}$, then pick any $N$ jobs out of total $n_\iota(t)$ jobs.}  that are in their in-elastic phase, and among the $n_e(t)$ jobs  that are in their elastic phase, 
process the $\beta n_e(t)$ that have arrived {\bf most recently}.
{\bf Speed:} 
\begin{align}\label{}
  s(t) & = \begin{cases} 1 & \text{for each of}  \min\{n_\iota(t),N\} \ \text{jobs}, \\ 
  P\left(\frac{N-\min\{n_\iota(t),N\}}{\beta n_e(t)}\right) & \text{for each of} \ \beta n_e(t) \ \text{jobs}.\end{cases}
\end{align}
IIb:If $n_\iota(t) < \theta n(t)$ Among the $\beta n(t)$ jobs that have arrived {\bf most recently},  process all the jobs that are in their elastic phases with equal speed
\begin{align}\label{}
  s(t) & =  P\left(\frac{N}{ \beta n(t)}\right). 
\end{align}
Note that in this subcase, the total speed  
constraint of $\sum_{j= 1}^{A(t)} P^{-1}(s_j(t)) \leq N$ need not be tight. Thus, for a practical implementation, few more jobs can be processed, however, 
that will not change the analysis.

By its very definition, algorithm \textsc{Fractional-LCFS} satisfies the total speed  
constraint of $\sum_{j= 1}^{A(t)} P^{-1}(s_j(t)) \leq N$, as well as the speed constraint of unity for any job that is in its in-elastic phase.

The main result of this paper is as follows.
\begin{theorem}\label{thm:flowtimeplusenergyonline}
  For any $\alpha > 1$, there exists a $0 < \theta < \beta < 1$, such that the competitive ratio of algorithm \textsc{Fractional-LCFS} for Problem \eqref{eq:flowtime} is a constant (depends only on $\alpha$) and is independent of the number of jobs, their sizes, and the number of servers $N$. The exact competitive ratio 
  expression is provided in \eqref{eq:finalbound}, and using which for example in case of $\alpha=2$, we get the competitive ratio bound of $636$, choosing $\beta = \frac{1}{6}$, and $\theta= \frac{1}{72}$.\end{theorem}

For each value of $\alpha>1$, how to choose $\beta,\theta$ such that the competitive ratio remains a constant is discussed in Remark \ref{rem:choiceofbeta}. Note that in Remark \ref{rem:choiceofbeta} we  prescribe only one possible choice of parameters $ \theta, \beta$ that is sufficient to make the competitive ratio as a constant. However, there is scope for choosing the parameters $ \theta, \beta$ so as to minimize the competitive ratio, which is analytically challenging, but easy numerically.


\begin{remark}\label{}
  It is worth noting that the competitive ratio bound in Theorem \ref{thm:flowtimeplusenergyonline} increases as $\alpha \rightarrow 1$. The main intuition for this is that we are considering the worst case input, which includes the case where jobs have no in-elastic phases, for which as $\alpha \rightarrow 1$, SRPT is an optimal algorithm that processes only one job 
  with the least remaining size on all servers. In contrast, with \textsc{Fractional-LCFS}, potentially a large number of jobs are parallely processed with equal speed for all values of $\alpha$. 
\end{remark}

{\it Discussion:} 
%Theorem \ref{thm:flowtimeplusenergyonline} shows that a simple LCFS algorithm that processes a fraction of the most recently arrived outstanding jobs, that is 
%not even aware of the remaining job size (of any remaining phase) and that uses equal 
%speed for jobs that are in the same phase, is constant competitive, i.e., independent 
%of input parameters: number of jobs and their sizes, and the number of servers, and 
%only depends on the speedup exponent $\alpha$. 
Even though the derived competitive ratio of  \textsc{Fractional-LCFS} appears large, it overcomes an
old technical hurdle of it being independent of system parameters.
In prior work, either speed augmentation \cite{edmonds2000scheduling} was shown to be necessary to get similar
constant competitive ratio results, or somewhat simplistic input model 
had to be considered \cite{berg2021case}. Moreover, given the very nature of the competitive ratio metric being a multiplicative penalty, a large competitive ratio per se is not limiting, as long as it does not scale with system parameters.


The intuition as to why a fractional LCFS algorithm should perform well  is similar to that of 
the SRPT (shortest remaining processing time) algorithm that requires the knowledge of remaining job sizes. 
SRPT minimizes the number of outstanding jobs (that controls the flow time) knowing the jobs sizes, by keeping 
shorter jobs in the system for less time. Fractional LCFS on the other hand, without using the remaining job size information, 
processes a fraction of the most recently
arrived jobs, and tries to keep  longer jobs stay in the system for long, thus `effectively' prioritizing short jobs. It is easy to construct 
`bad' input sequences where this is not the case, but roughly that is what one should expect.

%The speed choice made by the proposed algorithm is primarily dictated by the constructed potential function and the unity speed constraint for the in-elastic phase, so 
%that the overall drift (derivative) of the potential function is sufficiently large. In particular, the speed chosen for 
%jobs that are in the same phase is always identical. 
Moreover, the intuition for the equal speed choice can be 
borrowed from \cite{edmonds2000scheduling}, that explains that if an algorithm choosing equal speed has more number of 
outstanding jobs than the $\opt$, then 
progressively, it allocates fewer servers to each job and since $\alpha >1$, it improves the utilization 
of servers. Since we also have jobs that are in their in-elastic phase, this is not precisely correct, however, provides partial 
explanation. 




%\begin{corollary}\label{cor:equalsizejobs}
%  The competitive ratio of \textsc{PA-EQUI} for Problem \eqref{eq:flowtimeplusenergy} when all jobs are of equal size, is a constant. 
%\end{corollary}
%\begin{proof} Let $n(t)$ be the number of outstanding jobs with any algorithm $\cA$ and \textsc{PA-EQUI} at time $t$. Then 
%since with EQUI, all outstanding jobs are processed with equal speed, the amount of work done (sum of the processed job sizes) in time $[t, t+dt]$ with \textsc{PA-EQUI} is more than $\cA$, in particular the \textsc{Fractional-LCFS} algorithm. 
%Moreover, since all jobs are of same size, a newly arrived job that will get start getting processed by \textsc{Fractional-LCFS} algorithm has a larger size than all the outstanding jobs with EQUI. 
%\end{proof}



After dealing with the setting where jobs arrive at arbitrary times, next, we consider the simpler case when all jobs are available at time $0$ and get a better competitive ratio 
guarantee.

\section{All jobs available at time $0$} In this section, except for all jobs arriving at time $0$, everything is identical to the system model described in Section \ref{sec:sysmodel}.
%We show that a simpler algorithm, called EQUI, that processes all jobs simultaneously at the same speed, and does not require the knowledge of remaining job sizes, has a  constant (depending on $\alpha$) competitive ratio for both Problem \eqref{eq:flowtime} and Problem \eqref{eq:flowtimeplusenergy}. 
For this case, we propose an algorithm  \textsc{PA-EQUI} that makes the following choice for scheduling and speed selection.

Case I $\frac{N}{n(t)} \le 1$: Process all the $n(t)$ (number of outstanding) jobs, without distinguishing between jobs that are in their elastic or in-elastic phase, with equal speed $  s(t)  = P\left(\frac{N}{n(t)}\right).$


Case II $\frac{N}{n(t)} > 1$: 
IIa: For a constant $0 < \delta < 1$, if $n_\iota(t) \ge \delta n(t)$ then process all $n_\iota(t)$ jobs  that are in their in-elastic phase dedicatedly in one server with unit speed, while process the remaining  $n_e(t)$ jobs that are in their elastic phase, each with speed $P\left(\frac{N-n_\iota(t)}{ n_e(t)}\right)$.

IIb:If $n_\iota(t) < \delta n(t)$ Process all the $n_e(t)$ jobs that are in their elastic phase, each with equal speed $  s(t)  =  P\left(\frac{N}{n_e(t)}\right)$.
We name this algorithm \textsc{PA-EQUI}, since it allocates equal speed to all jobs that belong to the same phase. In contrast, \textsc{EQUI} studied in \cite{edmonds2000scheduling,edmonds2009scalably}
 is \textsc{Blind-EQUI}, since it is unaware which jobs belong to which phase, and wastes speed. 
By its very definition, algorithm \textsc{PA-EQUI} satisfies the total speed  
constraint of $\sum_{j= 1}^{A(t)} P^{-1}(s_j(t)) \leq N$, as well as the speed constraint of unity for any job that is in its in-elastic phase.

The main result of this section is as follows.
\begin{theorem}\label{thm:flowtimetimezero}
  For $\alpha >1$, the competitive ratio of \textsc{PA-EQUI} for Problem \eqref{eq:flowtime} when all jobs are available at time $0$, is at most $$\mu(\alpha) = \frac{1}{\alpha(1-\delta)-1}\left[\frac{\alpha(1-\delta)}{\delta} + \frac{\alpha(1-\delta)+\delta}{1-\delta}\right],$$
  where $\delta$ is the parameter to be chosen. 
  For $\alpha=2$, choosing $\delta=\frac{1}{4}, \mu(2) = 50/3$. 
  Moreover, $\mu(\alpha)$ is a decreasing function of $\alpha > 1$ for an appropriate choice of $\delta$.
\end{theorem}
Proof is similar to that of Theorem \ref{thm:flowtimeplusenergyonline} and for lack of space is omitted. It can be found in the full version \cite{fullversion}.
Thus, compared to the online job arrivals case (Theorem \ref{thm:flowtimeplusenergyonline}) where the competitive ratio for $\alpha=2$ is $636$,
there is a significant improvement in the competitive ratio when all jobs are available at time $0$. Similar conclusion can be drawn for other values of $\alpha$ also.
%From the Theorem we conclude that as $\alpha$ approaches $1$ the competitive ratio worsens and at $\alpha=1$ it is unbounded. This is similar to negative result  which in line with the 
%lower bound of $n^{1/3}$ for any no
%To prove Theorem \ref{thm:flowtimetimezero}, similar to the previous section, we consider the following potential function, and show that  \eqref{eq:runcond} holds for 
%a particular value of $\kappa$.

\begin{comment}
{\bf Potential Function} 
At time $t$, let $A(t)$ be the set of unfinished jobs with \textsc{PA-EQUI}  where $n(t) = |A(t)|$, and for the $i^{th}$ job,  $i\in A(t)$, let $q_i(t)$ be its remaining (sum of remaining sizes of all the remaining phases) size. Then  
\begin{align}\label{}
 n^i(t,q) & = \begin{cases} 1 & \text{for} \  q\le q_i(t), \\
 0 & \text{otherwise.}
 \end{cases}
\end{align} 
Similarly, let $n_o(t)$ be the number of unfinished jobs with the $\opt$, and the corresponding quantity to $n^i(t,q)$ for the $i^{th}$ job with the $\opt$, be denoted by $n^i_o(t,q)$. 




Consider the potential function
\begin{equation}\label{defn:phispecialFT}
\Phi^{sf}(t) = c_1\Phi^{sf}_1(t) + c_2\Phi_2(t),
\end{equation}
where 
\begin{equation}\label{defn:phi1specialFT} 
\Phi^{sf}_{1}(t) =  P\left(\frac{n(t)}{N}\right) \left(\sum_{i\in A(t)}\int_{0}^\infty ( n^i(t,q) - n^i_o(t,q))^+ dq\right),
\end{equation}
where $c_1$, and $c_2$ are constants to be chosen later, and $(x)^+ = \max\{0,x\}$, and $\Phi_2(t)$ is as defined in \eqref{phi2}.

Clearly, $\Phi^{sf}(t)$ satisfies the first boundary condition. 
Since all jobs are available at time $0$, which is equivalent to all arrivals happening at time $t=0$, both $\Phi^{sf}_{1}(t)=0$ and $\Phi_2(t)=0$ for $t=0$. Thus, to check whether $\Phi^{sf}(t)$ satisfies the second boundary condition, 
we only need to check whether $\Phi^{sf}(t)$ increases on a departure of a job with either the \textsc{PA-EQUI} or the $\opt$.
\begin{lemma}\label{lem:jumpequi}
Potential function $\Phi^{sf}(t)$ \eqref{defn:phispecialFT} does not increase on a departure of a job with either the \textsc{PA-EQUI} or the $\opt$.
\end{lemma}

The proof of Lemma \ref{lem:jumpequi} is provided in Appendix \ref{app3}.
Next, we characterize the drift $d \Phi^{sf}(t)/dt$.
\begin{lemma}\label{lem:driftphisopt}
Because of the processing by the $\opt$,  the change in the potential function \eqref{defn:phispecialFT} is
\begin{align*}
d \Phi^{sf}(t)/dt & \le   c_1 \left(\frac{1}{\alpha}\right) n(t) + c_1\left(1-\frac{1}{\alpha}\right) n_o(t) + c_2 n_o(t).
\end{align*}
\end{lemma}

The proof of Lemma \ref{lem:driftphisopt} is provided in Appendix \ref{app4}.
\begin{lemma}\label{lem:driftphisalg}
Because of the processing by the algorithm \textsc{PA-EQUI}, the change in the potential function \eqref{defn:phispecialFT} is
 \begin{align} 
 d\Phi^{sf}(t)/dt & \le \begin{cases} -c_1(\max\{n(t)-n_o(t),0\} )  &  \text{if} \ \frac{N}{ n(t)} \le 1, \\
  -c_2 n_\iota(t) &  \text{if} \ \frac{N}{ n(t)} > 1 \ \text{and} \ n_\iota(t) \ge \delta n(t),\\
  - c_1 (\max\{n_e(t)-n_o(t),0\} )& \text{if} \ \frac{N}{ n(t)} > 1 \ \text{and} \ n_e(t) \ge (1-\delta) n(t).
   \end{cases}
 \end{align}
\end{lemma}
The proof of Lemma \ref{lem:driftphisalg} is provided in Appendix \ref{app5}.
With these preliminaries, we are ready to prove  Theorem \ref{thm:flowtimetimezero}.
\begin{proof}[Proof of Theorem \ref{thm:flowtimetimezero}]
Case I : $\max\{n(t)-n_o(t),0\}  =0.$ In this case, we only count the $\opt$'s contribution to $d\Phi^{sf}(t)/dt$ from Lemma \ref{lem:driftphisopt}, since $d\Phi^{sf}(t)/dt$ because 
of \textsc{PA-EQUI}'s processing is always non-positive. Thus, we can write   \eqref{eq:runcond}, as 
\begin{align}\nn
n(t)  +   d\Phi^{sf}(t)/dt& \le n(t)   + c_1 \left(\frac{1}{\alpha}\right) n(t) + c_1\left(1-\frac{1}{\alpha}\right) n_o(t) + c_2 n_o(t), \\ \nn
& \le n_o(t)(1+c_1+c_2), \end{align}
where the second inequality follows since $n(t) \le n_o(t)$.
%where the last inequality follows since the $\opt$ has non-zero jobs i.e., $n_o(t) >0$, in which case the total power used by it $P^o_{\text{sum}}(t)=\bp$.

Case II: $n_o(t)> 0$,  $\max\{n(t)-n_o(t),0\} = n(t)-n_o(t)$, and $n(t) \ge N$.
Using Lemma \ref{lem:driftphisopt} and \ref{lem:driftphisalg}, we can write \eqref{eq:runcond},
\begin{align}\nn
 n(t)  +   d\Phi^{sf}(t)/dt& \le n(t)   + c_1 \left(\frac{1}{\alpha}\right) n(t) + c_1\left(1-\frac{1}{\alpha}\right) n_o(t) + c_2 n_o(t) -c_1(\max\{n(t)-n_o(t),0\} ), \\  \nn
  & \le n(t)\left(1+ c_1\left(\frac{1}{\alpha}\right)-c_1 \right) + n_o(t)\left(c_1\left(1+\left(1-\frac{1}{\alpha}\right)\right)+c_2\right),\\  \label{eq:runcond2}
  & \le n_o(t)\left(c_1\left(1+\left(1-\frac{1}{\alpha}\right)\right)+c_2\right),
\end{align}
for $ c_1\ge 1/\left(1-\left(\frac{1}{\alpha}\right)\right)$.

Case II: $n_o(t)> 0$,  $\max\{n(t)-n_o(t),0\} = n(t)-n_o(t)$,  $n(t) < N$  and $n_\iota(t) \ge \delta n(t)$.
Using Lemma \ref{lem:driftphisopt} and \ref{lem:driftphisalg}, we can write \eqref{eq:runcond},
\begin{align}\nn
 n(t)  +   d\Phi^{sf}(t)/dt& \le n(t)   + c_1 \left(\frac{1}{\alpha}\right) n(t) + c_1\left(1-\frac{1}{\alpha}\right) n_o(t) + c_2 n_o(t) -c_2 n_\iota(t), \\  \nn
  & \stackrel{(a)}\le n(t)\left(1+ c_1\left(\frac{1}{\alpha}\right)- \delta c_2 \right) + n_o(t)\left(c_1\left(1-\frac{1}{\alpha}\right)+c_2\right),\\  \label{eq:runcond2}
  & \le n_o(t)\left(c_1\left(1-\frac{1}{\alpha}\right)+c_2\right),
\end{align}
where $(a)$ follows since $n_\iota(t) \ge \delta n(t)$, and the final inequality follows
for $\delta c_2 \ge 1+\frac{c_1}{\alpha}$.

Case III: $n_o(t)> 0$,  $\max\{n(t)-n_o(t),0\} = n(t)-n_o(t)$,  $n(t) < N$  and $n_e(t) \ge (1-\delta) n(t)$.

Case IIIa: $\max\{n_e(t)-n_o(t),0\}  =0.$
 In this case, we only count the $\opt$'s contribution to $d\Phi^{sf}(t)/dt$ from Lemma \ref{lem:driftphisopt} since $d\Phi^{sf}(t)/dt$ because 
of \textsc{PA-EQUI} is always non-positive. Thus, we can write   \eqref{eq:runcond}, as 
\begin{align}\nn
n(t)  +   d\Phi^{sf}(t)/dt& \le n(t)   + c_1 \left(\frac{1}{\alpha}\right) n(t) + c_1\left(1-\frac{1}{\alpha}\right) n_o(t) + c_2 n_o(t), \\ \nn
& \le n_o(t)\left(\frac{1}{(1-\delta)}+c_1\left(1+\frac{\frac{1}{1-\delta}-1}{\alpha}\right)+c_2\right), \end{align}
where the second inequality follows since $n(t) \le \frac{n_o(t)}{1-\delta}$ as $n_e(t) \ge (1-\delta) n(t)$ and $\max\{n_e(t)-n_o(t),0\}  =0$.


Case IIIb: 
$\max\{n_e(t)-n_o(t),0\}  =n_e(t)-n_o(t).$
\begin{align}\nn
 n(t)  +   d\Phi^{sf}(t)/dt& \le n(t)   + c_1 \left(\frac{1}{\alpha}\right) n(t) + c_1\left(1-\frac{1}{\alpha}\right) n_o(t) + c_2 n_o(t) +c_1\left(-\max\left\{n_e(t)-n_o(t),0\right\}\right), \\  \nn
  & \stackrel{(a)}\le n(t)\left(1+ c_1\left(\frac{1}{\alpha}\right)-(1-\delta) c_1 \right) + n_o(t)\left(c_1\left(1+\left(1-\frac{1}{\alpha}\right)\right)+c_2\right),\\  \label{eq:runcond2}
  & \le n_o(t)\left(c_1\left(1+\left(1-\frac{1}{\alpha}\right)\right)+c_2\right),
\end{align}
where $(a)$ follows since $n_e(t) \ge (1-\delta) n(t)$, and the final inequality follows for
$ c_1\ge \alpha/\left(\alpha(1-\delta)-1\right)$.


When $n_o(t) =0$, then we get that \eqref{eq:runcond} holds with a smaller constant $\kappa$.

Combining, all the conditions, we get that the competitive ratio is at most $\left(\frac{1}{1-\delta}+c_1\left(1+\frac{\frac{1}{1-\delta}-1}{\alpha}\right)+c_2\right)$ where 
$c_1\ge \alpha/\left(\alpha(1-\delta)-1\right)$ and $\delta c_2 \ge 1+\frac{c_1}{\alpha}$. Thus, the tightest bound is

$$\left(\frac{1}{1-\delta}+c_1\left(1+\frac{\frac{1}{1-\delta}-1}{\alpha}\right)+c_2\right)$$ $$ \le \frac{1}{\alpha(1-\delta)-1}\left[\frac{\alpha(1-\delta)}{\delta} + \frac{\alpha(1-\delta)+\delta}{1-\delta}\right] .$$
\end{proof} 
\end{comment}
\input{SimulationResults.tex}

\section{Conclusions}
In this paper, we considered an important problem of flow time minimization in  data centers, where jobs migrate between two phases of parallelizability (called  elastic and in-elastic) multiple times. In the 
elastic phase, there is flexibility of parallelizing the job over multiple servers, while in the in-elastic phase, the job has to be processed by a single server. 
Moreover, in the elastic phase there is  limited parallelizability, and the speed increment diminishes as more and more servers are allocated to any job.
We considered the online setting, where jobs arrive over time with arbitrary sizes and arrival times, and proposed a LCFS type algorithm for scheduling,  that 
processes the  scheduled jobs with equal speed. We showed that  its competitive ratio is a constant that only depends on the speed-up exponent $\alpha$ as long as $\alpha>1$. 
%In recent work, this model has been considered, however, for a specific stochastic input, where the size of the job in both the elastic and the in-elastic phase was exponentially distributed with identical parameters in the two phases, and 
%a job always departed on completion of some in-elastic phase.
%With the specific stochastic input, always scheduling as many  jobs that are in their in-elastic phases was shown to be optimal. 
With arbitrary input, our result overcomes fundamental difficulty found in literature where similar results were shown only in the presence of resource augmentation or for simpler model, by exploiting the 
specific structure of the problem with just two phases that is practically well motivated. 
%We also considered the 
%case when all jobs are available at time $0$, and for which a different algorithm has significantly 
%better competitive ratio than the online jobs arrival case.
%The competitive ratio for most relevant speed-up exponents of $2$ and $3$, is at most 690, which even though large, does not depend on any parameters of the problems such as the number of jobs, or their job sizes, which is of primary importance. 
%This is a classical problem, where recently an optimal 
%increasing the number of servers assigned to any job increases its speed , but the i

% such that $\frac{(1-\beta) (\beta - \gamma) }{\beta} > 1/2$. 
%while keeping $\frac{1+c/2}{\gamma}$ as small as possible where $c =  \frac{2}{\frac{(1-\beta) (\beta - \gamma) }{\beta} - 1/2}$. 
  
% Recall that $\beta = \frac{1}{4}$. Let the choice of  $\gamma$ be $\gamma = \beta ^2$. Then $\frac{(1-\beta) (\beta - \gamma) }{\beta} = (3/4)^2 > 1/2$, and choice of $c$ that satisfies both \eqref{eq:condfirstc} and \eqref{eq:condsecc} is  $$c= \frac{2 (P(4)/4)}{\frac{(1-\beta) (\beta - \gamma) }{\beta} - 1/2}.$$
%
%  %Let $\gamma = \beta ^2$. Then $\frac{(1-\beta) (\beta - \gamma) }{\beta} = (3/4)^2 > 1/2$. 
% With this choice of $c$, the competitive ratio is controlled by  \eqref{eq:c1}, and is given by 
% $$\frac{1+c/2}{\gamma} = 16 \left(1+ \frac{ (P(4)/4)}{\frac{(1-\beta) (\beta - \gamma) }{\beta} - 1/2}\right) < 16(1+ 16 P(4)/4).$$
  
% From Lemma \ref{lem:optpower}, $P^o_{\text{sum}}(t) = N$, whenever there is an outstanding job with the $\opt$.
%Since $N> 1$, $N/2+1 \le 3/2 N$. Thus, combining \eqref{eq:c1} and \eqref{eq:c2}, and using \eqref{eq:runcond}, the competitive ratio of the algorithm is at most $\kappa \le (1+c/2)/\gamma \le 17\times 16=272$.
%//

%\subsection{$N < \frac{P(4)}{4}$}
  
%Suppose $k$ jobs arrive over time $[t_0, t)$, and let $m$ of them depart with the $\opt$. Thus, $n_o \ge k -m $
%The maximum speed that  $\opt$ can give to any job is $P(N)$, while the maximum speed that the algorithm gives to any job is $P(N/n(t))$. Thus, at least $m/
  
  %Claim Which is Not TRUE
%  \begin{lemma}\label{}
%  Claim $n(t) \le n_o(t) + N + P(n(t))$.
%\end{lemma}
%
%\begin{proof}
%Let at some time  $t$, $n(t) > N$, since otherwise the claim is always true. Then consider the latest time $t_0< t$, when $n^\cA(t_0) = N$. We will focus on interval $[t_0, t)$. 
%Let the $\opt$ work on one job with speed $P(N)$ during $[t_0, t)$.  This will ensure maximum number of departures happen in $[t_0, t)$ for the $\opt$. Let the number of new jobs that arrive during $[t_0, t)$ be $k$, while the number of departures be $m$ during $[t_0, t)$ with the $\opt$. 
%
%Then $n_o(t) \ge k-m$.
%
%Let there be no departure with the algorithm during the interval $[t_0, t)$ (worst case). 
%With no departures between time $[t_0, t)$, the speed dedicated by the algorithm to any job throughout the duration $[t_0, t)$ is at least $P(N/n(t))$. Before the first departure with the algorithm, the maximum number of departures that can happen with $\opt$ is at most 
%$P(n(t))$. Thus, $m \le P(n(t))$. 
%
%Putting all this together, we get 
%$$n(t) \le n^\cA(t_0) + k \le N + n_o(t) + m \le N + n_o(t) +P(n(t)),$$
%as required.
%
%
%\end{proof}


